A Systematic Literature Review on Reasons and Approaches for Accurate Effort Estimations in Agile

Background: Accurate effort estimation is crucial for planning in Agile iterative development. Agile estimation generally relies on consensus-based methods like planning poker, which require less time and information than other formal methods (e.g., COSMIC) but are prone to inaccuracies. Understanding the common reasons for inaccurate estimations and how proposed approaches can assist practitioners is essential. However, prior systematic literature reviews (SLR) only focus on the estimation practices (e.g., [26, 127]) and the effort estimation approaches (e.g., [6]). Aim: We aim to identify themes of reasons for inaccurate estimations and classify approaches to improve effort estimation. Method: We conducted an SLR and identified the key themes and a taxonomy. Results: The reasons for inaccurate estimation are related to information quality, team, estimation practice, project management, and business influences. The effort estimation approaches were the most investigated in the literature, while only a few aim to support the effort estimation process. Yet, few automated approaches are at risk of data leakage and indirect validation scenarios. Recommendations: Practitioners should enhance the quality of information for effort estimation, potentially by adopting an automated approach. Future research should aim to improve the information quality, while avoiding data leakage and indirect validation scenarios.

==> litrev_section_result2.tex <==
\section{Results}\label{sec:litrevresult}

In this section, we provide an overview on the search results and describe our findings for each research question.

\subsection{Search Results}

Based on our search in March 2022, \litrevtotalpaper{} studies passed the inclusion, exclusion, and quality criteria screening.
From the \litrevtotalpaper{} selected studies, \litrevreasonspaper{} of them investigating the \reasons{} (IC-4A) and \litrevapproachpaper{} of them proposed an approach for effort estimation (IC-4B).
Noted that we found two studies satisfied both IC-4A and IC-4B.
Figure~\ref{fig:litrevapproach} shows the number of the studies that passed each study selection phases.
Majority of these studies were published after year 2016 (see Figure~\ref{fig:publishedyear}).
Below, we describe the detail of the three screening phases.


\textbf{In phase A,} \litrevphaseascreening{} studies passed the screening by applying the inclusion criteria on the title and abstract of the study.
Figure~\ref{fig:litrevapproach} shows the number of studies that passed the three study selection phases. 
On the other hand, 58 and 128 studies were not satisfied IC-3 and IC-4, respectively.
Noted that no study was excluded due to IC-1 and IC-2 since we filtered them out during the search process.
When examining the title and abstract, we could not determined whether 21 studies satisfied IC-4 due to insufficient information.
We further considered the introduction, background, and conclusion of these studies.
Finally, nine of these studies satisfied IC-4A or IC4-B.
In summary, \litrevphaseascreening{} studies passed phase A screening.
In addition, we revisited all studies that were related to Agile context (IC-1) but not satisfied IC-4.
We found that they are related to software quality and testing (41 studies), development practices (33 studies), human aspect (20 studies), Agile adoption (17 studies), requirements engineering (13 studies), and others (23 studies).

\textbf{In phase B,} \litrevphasebscreening{} studies passed the screening based on the inclusion and exclusion criteria.
Particularly, 8 studies were excluded due to no access provided (EC-1).
We contacted the developers but there was no response.
After that, we excluded 7 duplicate studies or continuation of the other included studies (EC-2), 13 literature review studies (EC-3), 7 experience report or replication studies (EC-4), and 22 studies that evaluated the existing effort estimation techniques.
Noted that no study was excluded when we re-applied the inclusion criteria again in full text.

\textbf{In phase C,} \litrevselected{} studies passed all the quality criteria.
Most of the excluded studies were excluded because there was no evaluation or validation methods described (QC-3).
However, we could not digest the number of the excluded studies per each criteria since we stopped reading when one of the five criteria was not satisfied.



\begin{figure}
\centering
\begin{subfigure}{.34\textwidth}
    \includegraphics[width=1\linewidth]{figures/litrev_yearRQ1.pdf}
    \caption{The selected studies that investigated the \reasons{}}
    \label{fig:publishedyearRQ1}
\end{subfigure}
\begin{subfigure}{.56\textwidth}
    \includegraphics[width=.95\linewidth]{figures/litrev_yearrq2}  
    \caption{The selected studies that proposed an approach to help the Agile practitioners estimate effort more accurate}
    \label{fig:publishedyearRQ2}
\end{subfigure}
\caption{The number of selected studies published in each year.}
\label{fig:publishedyear}
\end{figure}

\subsection{RQ1: \litrevrqone{}}

\input{tables/table_litrev_result_reasons_minimal}
 
In this RQ, we aim to better understand the common \reasons{} in Agile.
We identified \litrevreasonspaper{} studies that investigated the \reasons{}.
Table~\ref{tab:table_litrev_reasons} lists the \reasons{} reported by the seven selected studies that satisfied the IC-4A criterion.
We also retrieved the ranking of each reason from the selected studies (see Section~\ref{sec:litrevrankingmethod}).
The reasons were ranked based on the number of answered participants~\cite{usman2015effort, Britto2015}, the occurrences reported by the developers~\cite{conoscenti2019combining}, and the mean value of agreement provided by the participants~\cite{usman2018developing}.
% While most of the \reasons{} were reported in three studies or fewer, there are three reasons that were most frequently reported, i.e., lack of detail or unclear documentation (R1.1; 5/7 studies), unstable documentation (R1.2; 4/7 studies), and lack of experience on the technology or context (R2.1.1, 5/7 studies).
Based on our card sorting process, we identified six themes of the \reasons{}, i.e., \litrevreasonqualitylarge{} (R1), Team-related (R2), Estimation Practice (R3), Project Management (R4), Business Influence (R5), and Others (R6), which are described below.

\textbf{(R1) \litrevreasonqualitylarge{}: }
Quality of the available information was frequently reported as one of the common \reasons{} (also reported with the highest ranking).
The selected studies reported that, with the poor quality of the available information, the team may inaccurately anticipated the effort to implement a desired functionality~\cite{conoscenti2019combining, Britto2015}.
They also discussed that the changes or new work were late discovered during the implementation.
% In particular, several studies reported that poor documentation could lead to unpredicted activities during the estimation.
% During the implementation, the team may discover that the story needs more or less effort than the estimation during planning.
Based on our card sorting process, we identified three aspects of the information quality issues that impact the estimation accuracy, i.e., unclear information (R1.1), unstable information (R1.2), or error in the information (R1.3).
Unclear information (R1.1) refers to the lack of detail or unclear information during effort estimation (e.g., user stories, acceptance criteria, requirements)~\cite{conoscenti2019combining, sandeep2022effort, usman2018effort, usman2015effort, Britto2015}.
Conoscenti et al.~\cite{conoscenti2019combining} described that the understandability problems or unclear definition of the available information (e.g., user acceptance criteria) would lead to inaccurate estimation.
Unstable information (R1.2) refers to the available information that is keep changing or changed after the estimation was done, thus may affect the estimation accuracy~\cite{sandeep2022effort, usman2018effort, usman2015effort, Britto2015}.
Usman et al.~\cite{usman2015effort} reported that both changing the existing and introducing new requirements were the top reasons for effort overruns.
Error in the information (R1.3) refers to the requirements~\cite{Britto2015} or estimated effort~\cite{conoscenti2019combining} that were mis-documented.
Britto et al.~\cite{Britto2015} noted that mis-documented requirements could lead to unpredicted activities during the estimation process.
For the estimation errors, Conoscenti et al.~\cite{conoscenti2019combining} reported that an error in the estimation logging could simply cause the inaccurate estimations.


These information quality issues could be implied to any level of information.
In particular, three studies reported these reasons using the term ``requirements'', which could be implied to either a higher-level information~\cite{sandeep2022effort, usman2018effort, Britto2015}.
Other two studies reported the reasons based on Agile artifacts (lower-level), i.e., unclear user acceptance criteria~\cite{conoscenti2019combining} and poorly-specified user stories~\cite{usman2015effort, sandeep2022effort}.
% Sandeep et al.~\cite{sandeep2022effort} also reported the reason ``poor user stories'', however, the detail was not provided.
These observations suggest that poor information quality, either higher or lower level, could be the reason for inaccurate estimations.
% Aside from the description of the work to be done, Conoscenti et al.~\cite{conoscenti2019combining} pointed out that a simple mistake in logging the estimated effort (R1.3.2) could be another reason for an inaccurate estimation.


% These documentation quality problems may be due to the low-priority documentation principles of Agile principles~\cite{fowler2001agile}.

\textbf{(R2) \litrevreasonteamlarge{}:}
Many \litrevreasonteam{} issues were reported as the \reasons{}.
The \litrevreasonteam{} issues may affect the ability of the team to estimate the effort.
Based on our card sorting process, we identified four aspects of the \litrevreasonteam{} issues, including the lack of experience of team members (R2.1), insufficient stakeholders participation (R2.2), knowledge sharing problem (R2.3), and dominant personality (R2.4).
The lack of experience of team members (R2.1) refers to the lack of experience on the technology, domain knowledge, and effort estimation practices~\cite{conoscenti2019combining, sandeep2022effort, usman2015effort, Britto2015}.
This also includes on-boarding novice team members~\cite{conoscenti2019combining, sandeep2022effort, usman2018effort, usman2015effort} and the team with low cohesion (i.e., the team worked little time together)~\cite{Britto2015}.
Britto et al.~\cite{Britto2015} and Conoscenti et al.~\cite{conoscenti2019combining} reported that these issues might lead to a wrong assumption of the size of functionality or the team's ability to deliver, which affect the effort estimation accuracy.
Insufficient stakeholders participation (R2.2) covers the absent of three stakeholders during the estimation process.
First, the effort is not estimated by the development team~\cite{Britto2015}.
Second, the clients are not participating the estimation session to provide the details~\cite{usman2015effort, sandeep2022effort} or the effort was estimated considering an active participation of the clients (which in turn they did not)~\cite{Britto2015}.
Third, the scrum master is not guiding the team~\cite{sandeep2022effort,usman2015effort}.
Knowledge sharing problem (R2.3) refers to the problems in knowledge sharing.~\cite{usman2015effort,sandeep2022effort, vetro2018combining}.
Usman et al.~\cite{usman2015effort} pointed out that knowledge sharing and management problems should be considered in the estimation and managed during the execution.
Vetro et al.~\cite{vetro2018combining} reported that estimating new user stories without an explicit and shared reflection on the previous estimations could lead to inaccurate estimations.
Lastly, dominant personality (R2.4) refers to a team member with dominant personality that could influence the team estimations~\cite{sandeep2022effort}.
Since these team-related issues could lead to wrong assumptions during the estimation, these issues should be considered in the estimation and managed during the development to mitigate the impact on the estimation accuracy~\cite{usman2015effort, Britto2015}.


\textbf{(R3) \litrevreasonestimationlarge{}:}
Different issues related to the \litrevreasonestimation{} (R3) were reported as the \reasons{}.
% Prior work reported that poor estimation practices in several aspects could lead to inaccurate estimations.
Based on our card sorting process, we identified four aspects of the estimation practice issues reported by the selected studies, i.e., factors overlooked (R3.1), unnecessary work considered (R3.2), lack of formal estimation process (R3.3), and inappropriate estimation scale (R3.4).
Factors overlooked (R3.1) refers to when the team did not consider the factors or work in the estimation but they eventually have to work on them.
In the estimation session, the team overlooked side tasks~\cite{conoscenti2019combining}, overlooked non-functional requirements~\cite{sandeep2022effort, usman2015effort}, under-estimated the complexity of a developing function~\cite{conoscenti2019combining, usman2018effort}, ignored test effort~\cite{sandeep2022effort, usman2015effort}, was not aware of technical problems~\cite{conoscenti2019combining}, and assumed that a standard function is usable (which in turn it was not)~\cite{conoscenti2019combining}.
In contrast, considering unnecessary work (R3.2) refers to when the team considered some work in the estimation but it is not needed or already available.
The reported unnecessary work are the features or bug fixes that were not required for the user story~\cite{conoscenti2019combining}, the duplicate or redundant features that supposed to be done by other user stories~\cite{conoscenti2019combining}, the function that was over-estimated in terms of complexity~\cite{conoscenti2019combining, usman2018developing}, or the standard function that was in the development plan but already available~\cite{conoscenti2019combining}.
% Furthermore, Conoscenti et al.~\cite{conoscenti2019combining} pointed out that  considered small and should not cause much time (e.g., side tasks, testing effort, 
% Usman et al.~\cite{usman2015effort} also suggested that the accuracy could be improved if the user stories are well-understood.
Lack of formal estimation process (R3.3) refers to when the team did not follow a formal or structured estimation process~\cite{sandeep2022effort, usman2015effort}, i.e., the team performed ad-hoc estimations without following a formal estimation process like Planning Poker.
This seems to be counter-intuitive as Agile prefer interactions among people over processes and tools~\cite{fowler2001agile}.
However, Usman et al.~\cite{usman2015effort} argued that the estimation process should be aligned with Agile philosophy but not completely ignored.
Inappropriate estimation scale (R3.4) refers to the usage issues of the estimation scale.
Tamrakar et al.~\cite{tamrakar2012does} found that the adoption of the Fibonacci estimation scale could lower the estimation accuracy.
However, Vetro et al.~\cite{vetro2018combining} argued that using a numerical scale many not guarantee a good accuracy. 
Vetro et al.~\cite{vetro2018combining} reported that having too many items in the estimation scale or using a misleading numerical scale could lead to wrong estimations.

\textbf{(R4) \litrevreasonprojectlarge{}:}
Issues related to \litrevreasonproject{} (R4) were reported as the \reasons{}.
Based on our card sorting process, we identified three aspects of the project management issues, i.e., overhead due to distributed team settings (R4.1), poor change management (R4.2), and poor human-resource management (R4.3).
Overhead due to distributed team settings (R4.1) refers to the communication overhead when the team is working across multiple sites.
Britto et al.~\cite{Britto2015} and Sandeep et al.~\cite{sandeep2022effort} reported that the time, language, cultural differences, and the distances to the client affect the team communication, which may lead to inaccurate estimations if the communication overhead is not properly considered.
Complementing this finding, Usman et al.~\cite{usman2018effort} reported their analysis based on six product customization that the work being done in multiple sites tend to have a stronger underestimation.
Poor change management (R4.2) refers to when the scope of work was changing (i.e., scope creep) due to poor change control.
Sandeep et al.~\cite{sandeep2022effort} and Usman et al.~\cite{usman2015effort} reported that these issues may negatively impact the development time and project cost.
Poor human resource management (R4.3) refers to the delays due to the dependence on external resources~\cite{conoscenti2019combining, usman2018effort}, unavailability of the developers~\cite{conoscenti2019combining}, and turnover issues~\cite{usman2015effort, karna2020effects}.
However, we observed a disagreement on the turnover issues.
Usman et al~\cite{usman2015effort} reported that a high employee turnover would affect the estimation accuracy.
On the other hand, Karna et al.~\cite{karna2020effects} reported that not all turnover can have a negative impact on the estimation accuracy, while unplanned turnover can have a significant negative impact on the reliability of the expert estimation.


\textbf{(R5) \litrevreasonbusinesslarge{}:}
\litrevreasonbusinesslarge{} issues (R5) were reported as the \reasons{}.
Based on our card sorting process, we identified two aspects of the business influence issues, i.e., overoptimism due to project bidding pressure (R5.1) and pressure of timeline (R5.2).
Overoptimism due to project bidding pressure (R5.1) refers to when the team intentionally under-estimate the effort by considering only best case scenario to obtain a contract~\cite{usman2015effort, sandeep2022effort}.
Usman et al.~\cite{usman2015effort} also argued that such unfair practice could be a breach of the code of ethics for software engineers~\cite{gotterbarn1999computer}.
Pressure of timeline (R5.2) was reported by Sandeep et al.~\cite{sandeep2022effort} as one of the reasons for the inaccurate estimations.
However, no further explanation was provided.

\textbf{(R6) Others:}
There were two other \reasons{}.
Conoscenti et al.~\cite{conoscenti2019combining} reported that a story may be rejected by the reviewer during the code review process (R6.1), causing the team to take more time than expected.
Sandeep et al.~\cite{sandeep2022effort} reported that hardware problem (R6.2) may also affect the estimations.
However, no further detail was given for this reason.


\resultBox{
    \textbf{Findings:} The \litrevreasonqualitysmall{} are the common \reasons{} reported in selected studies
    The reasons in this theme were reported with a generally higher ranking than the others.
    The reasons in other theme, i.e., team-related, estimation practice, project management, business influence, were also reported, however, in a lower ranking.
    
    \textbf{Implication:} Poor quality of the available information are the common reason for inaccurate effort estimation.
}


\subsection{RQ2: \litrevrqtwo{}}


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figures/litrev_rq2categorization.pdf}
    \caption{Categorization of the \approaches{} based on the purposes of the approaches and planning levels.}
    \label{fig:litrevrq2}
\end{figure}

In this RQ, we identified \litrevapproachpaper{} studies proposed the \approaches{} in Agile.
Figure~\ref{fig:litrevrq2} shows that we categorized these approaches based on their purposes into two groups, i.e., (1) \purposeestimate{} and (2) \purposesupport{}.
To provide additional context on the approaches, we further categorized the approaches based on the planning level they designed to be used for.
Below, we discuss these approaches based on their purposes and planning levels.


% Commonly, an Agile team relies on expert judgement or team consensus to estimate the effort~\cite{Usman2016}.
% Despite their lower accuracy~\cite{dantas2018effort}, these approaches are widely-used as they are lightweight and easy to adopt~\cite{rubin2012essential, Cohn2006, Usman2016}.
% As shown in Figure~\ref{fig:litrevrq2}, we categorized the selected studies based on their purposes into two groups, i.e., (1) \purposeestimate{} and (2) \purposesupport{}.
% Next, we discuss the selected studies in each group.


\input{tables/table_litrev_result_approachestimation}


\subsubsection{\textbf{\purposeestimatelarge}} 
Table~\ref{tab:table_litrev_result_approachestimation} listed \litrevestimatepaper{} studies that proposed the approaches to ``\purposeestimate{}'' during sprint planning, project planning, project bidding, and maintenance.
% These approaches applied machine learning-based, parametric-based, or manual techniques to \purposeestimate{}.
Since effort estimation in Agile focuses on the sprint planning level~\cite{Usman2014, rubin2012essential, Cohn2006}, we discuss below the approaches to \purposeestimate{} during sprint planning, during other planning levels (i.e., project planning, project bidding, and maintenance), and the approaches that did not explicitly specify the planning level.

\subsubsubsection{\textbf{Sprint planning level}} 
% During sprint planning, the estimated effort is used when allocating the \wis{} to the sprint to ensure that their size fit the sprint capacity.
We observed that \litrevestimateforsprintplanning{} approaches aimed to \purposeestimate{} of \wis{} or sprints for (or during) sprint planning.
Majority of these approaches applied machine learning-based approaches to \purposeestimate{} (i.e., machine learning model~\cite{Porru2016, moharreri2016cost, scott2018, dantas2019effort, ramessur2021predictive}, neural network~\cite{Choetkiertikul2019, dragicevic2017bayesian} ensemble-based model~\cite{malgonde2019ensemble}, and fuzzy logic~\cite{alostad2017fuzzy}.
Three 



 \cite{Porru2016, moharreri2016cost, alostad2017fuzzy, dragicevic2017bayesian, scott2018, malgonde2019ensemble, dantas2019effort, Choetkiertikul2019vetro2018combining, altaleb2020pair, alhamed2021playing} & ML~\cite{ramessur2021predictive}, Parametric~\cite{kang2010model} 

 \cite{Porru2016, moharreri2016cost, alostad2017fuzzy, dragicevic2017bayesian, scott2018, malgonde2019ensemble, dantas2019effort, Choetkiertikul2019}, Manual \cite{vetro2018combining, altaleb2020pair, alhamed2021playing} & ML~\cite{ramessur2021predictive}, Parametric~\cite{kang2010model} 

We observed that \litrevestimateforsprintplanning{} of them were proposed to estimate the effort of \wis{} or sprints using machine learning-based techniques~\cite{Porru2016, moharreri2016cost, alostad2017fuzzy, dragicevic2017bayesian, scott2018, malgonde2019ensemble, dantas2019effort, Choetkiertikul2019, ramessur2021predictive}, parametric-based technique~\cite{kang2010model}, or manual techniques\cite{vetro2018combining, altaleb2020pair, alhamed2021playing}.
Furthermore, \litrevsupportforsprintplanning{} approaches were proposed to support the sprint planning by \litrevsupportcatonesmall{}~\cite{buglione2013improving, algarni2019applying}, \litrevsupportcattwosmall{}~\cite{usman2018developing, tanveer2019evaluation, tanveer2017utilizing, taibi2017operationalizing}, and \litrevsupportcatthreesmall{}~\cite{grapenthin2016supporting}.
These approaches were trained or evaluated using the information extracted from the \wis{} or sprints as the model inputs.
These inputs are related to the \wi{}, e.g., properties, summary and description, sprints, subtasks, experience and workload of developers, developing function, or other developers-provided inputs during sprint planning (e.g., Story Points or size estimated by an expert~\cite{moharreri2016cost, malgonde2019ensemble}).

However, the information (or requirements) related to \wis{} and sprints may be changed after sprint planning~\cite{hoda2016multilevel, jpsurvey, masood2020real}.
Yet, we observed that it is unclear whether these approaches (especially the ML-based ones) considered the uncertainty in the training or evaluation processes.
In other words, training or evaluating an effort estimation approach based on the completed and latest information may not reflect the usage scenario that the approaches were designed to be used for.
For example, Porru et al.~\cite{Porru2016} trained a Story Points estimation model based on the features of \wis{}.
They excluded the \wis{} with \infochgs{} or Story Points changes as the they may be unstable or contain misleading information.
We also observed that Malgonde and Chari~\cite{malgonde2019ensemble} considered the uncertainty by only train the model based on the types of information that are available during sprint planning.
Nevertheless, it is unclear whether the inputs of the prior proposed approaches were extracted from the information available during the sprint planning or not.
% These observations indicate that these proposed approaches may not fully perform during sprint planning.



\subsubsubsection{\textbf{Other levels}}

We identified \litrevestimateforotherlevels{} studies proposed an approach to estimate the effort for project planning, project bidding, and maintenance.
Five studies proposed the approaches to predict the effort for project planning~\cite{premalatha2019effort, panda2015empirical, raslan2018enhanced} and project bidding~\cite{parvez2013efficiency, rosa2017early}.
These studies used different techniques to overcome the lack of information problem in the early development stages.
For example, using the early design factors (e.g., risk resolution, team cohesion) as the model inputs~\cite{raslan2018enhanced}, using human-based estimations as the model inputs~\cite{panda2015empirical}, or evaluating the approach based on small sample sets~\cite{premalatha2019effort}.
Lastly, two studies proposed the approaches to predict the effort for software maintenance, i.e., phases in software maintenance~\cite{choudhari2012phase} and functional size of a change~\cite{sakhrawi2021support}.
% Lastly, Logue and Mcdaid~\cite{logue2008handling} proposed an approach that using a statistical simulation to help the team manage the uncertainty of the estimated effort in release planning.
% Choudhari and Suman~\cite{choudhari2012phase} used Planning Poker to estimate the Story Points of Requirement Change Stories before aggregating them to estimate the size of the maintenance phase.
% On the other hand, Sakhrawi et al.~\cite{sakhrawi2021support} used COSMIC functional size to predict the size of requirement changes and reported that their approach outperformed the Story Points-based approach.



\subsubsubsection{\textbf{Planning level not specified}}
We identified \litrevnotspecified{} studies proposed the approaches to \purposeestimate{} or \purposesupport{} but did not explicitly specified the planning level to be used for.
In particular, we identified \litrevestimatenotspecified{} studies proposed the ML-based approaches to \purposeestimate{} of a \wi{}~\cite{marapelli2020rnn, hemrajanipredicting, gultekin2020story, miranda2021analysis, dan2020nlp}, a sprint~\cite{Hearty2009, karna2020data}, a project~\cite{adnan2019ontology, bilgaiyan2019effort, khuat2018novel, farahneh2011linear, satapathy2014story, sharma2020linear, nunes2011iucp, ardiansyah2022mucpso}.
Other two studies proposed the parametric-based approaches to predict the effort of a requirement change~\cite{basri2016algorithmic} and a software increment~\cite{paz2014approach}.
For the approaches proposed to \purposesupport{}, only the study of Hannay et al.~\cite{hannay2019agile} did not specify the planning level for their approach.




\underline{\textit{Machine Learning-based:}} We identified 27 selected studies applied machine learning-based techniques to predict the effort.
In particular, these studies predict the effort using machine learning~\cite{Porru2016, moharreri2016cost, scott2018, dantas2019effort, ramessur2021predictive, sakhrawi2021support, hemrajanipredicting, gultekin2020story, karna2020data, adnan2019ontology, satapathy2014story, sharma2020linear, farahneh2011linear}, neural network~\cite{Choetkiertikul2019, premalatha2019effort, dragicevic2017bayesian, panda2015empirical, marapelli2020rnn, dan2020nlp, Hearty2009, bilgaiyan2019effort}, Practical Swarm Optimization~\cite{ardiansyah2022mucpso, khuat2018novel}, ensemble-based~\cite{malgonde2019ensemble}, fuzzy logic~\cite{alostad2017fuzzy}, and Monte Carlo simulation~\cite{miranda2021analysis} techniques.
% other automated techniques~\cite{ardiansyah2022mucpso, khuat2018novel, malgonde2019ensemble, alostad2017fuzzy, miranda2021analysis, alhamed2021playing} to predict the effort.
% Practical Swarm Optimization~\cite{ardiansyah2022mucpso, khuat2018novel}, ensemble-based~\cite{malgonde2019ensemble}, fuzzy logic~\cite{alostad2017fuzzy}, and Monte Carlo simulation~\cite{miranda2021analysis}.
We observed that the majority of these approaches used a supervised regression technique.
Only two approaches used a supervised classification technique to predict the effort, i.e., classifying Story Points in Fibonacci scale (Porru et al.~\cite{Porru2016}) and classifying the range of man-hours (Dan et al.~\cite{dan2020nlp}).
% Nevertheless, prior work reported that using a non-linear scale (e.g., Fibonacci scale) could lead an inferior prediction accuracy~\cite{tamrakar2012does}.

\underline{\textit{Parametric-based:}} We identified eight studies proposed algorithmic approaches to estimate the effort~\cite{choudhari2012phase, parvez2013efficiency, rosa2017early, nunes2011iucp, basri2016algorithmic, paz2014approach, kang2010model, raslan2018enhanced}.
We observed that these algorithmic approaches relies on the calculation based on Story Points~\cite{choudhari2012phase, raslan2018enhanced}, function points~\cite{paz2014approach, kang2010model}, use case points~\cite{parvez2013efficiency, nunes2011iucp}, and time units~\cite{rosa2017early, basri2016algorithmic}.

\underline{\textit{Manual:}} We identified two studies proposed the estimation methods that requires manual effort from an expert.
Vetro et al.~\cite{vetro2018combining} proposed an estimation process that adopted three major changes, i.e., using a shorter non-numerical estimation scale, comparing the estimation with the past user stories, and reviewing the past user stories that were inaccurately estimated.
Altaleb et al.~\cite{altaleb2020pair} proposed a pair-estimation technique that require a team member to estimate in pairs to create a deeper communication on the work to be done.
Lastly, Alhamed and Storer~\cite{alhamed2021playing} proposed a crowd-based estimation technique that simulates the Planning Poker estimation by recruiting the estimators from Amazon Mechanical Turk platform.
They reported that the crowd estimation achieved a similar accuracy as expert estimation with a lower cost.



% estimation techniques that require human effort, i.e., , combining both Story Points and COCOMO II estimation methods~\cite{raslan2018enhanced}, and using an algorithmic method to estimate the effort~\cite{choudhari2012phase, parvez2013efficiency, rosa2017early, nunes2011iucp, basri2016algorithmic, paz2014approach, kang2010model}.
% Nonetheless, relying on a prediction model with limited human involvement and transparency may hinder its adoption~\cite{minku2016data}.

\input{tables/table_litrev_result_approachsupport}

\subsubsubsection{\textbf{\purposesupportlarge{}}} 


We identified \litrevsupportpaper{} studies that proposed the approaches to \textit{``\purposesupport{}.''}
Specifically, these approaches are proposed to support the team decisions by \litrevsupportcatonesmall{}, \litrevsupportcattwosmall{}, and \litrevsupportcatthreesmall{}.
Table~\ref{tab:table_litrev_result_approachsupport} lists the approaches that were proposed to \purposesupport{}.
Majority of these approaches are manual (i.e., mainly or partly require the team effort to operate) and proposed to be used for (or during) sprint planning.

\underline{\textit{\litrevsupportcatone{}:}} Two approaches were proposed to improve the quality of the available information for effort estimation.
Buglione and Abran~\cite{buglione2013improving} proposed the use of INVEST criteria to improve the quality of user stories.
The process requires the team to determine whether a user story meet the INVEST criteria to improve the effort estimation accuracy.
Algarni and Magel~\cite{algarni2019applying} proposed a developer story artifact to provide technical information for the estimation.
The authors also demonstrated that the developer story could be used to trained a machine learning model to predict the story code size.

\underline{\textit{\litrevsupportcattwo{}:}}
Three approaches were proposed to identify additional information for effort estimation.
Usman et al.~\cite{usman2018developing} proposed a customized checklist to help the team recall relevant factors that should be considered during effort estimation.
They observed that the estimation accuracy of the teams is increased after using the checklist.
Nevertheless, as the checklist requires a lot of effort, the developers of a company opted-out due to its additional overhead.
Taibi et al.~\cite{taibi2017operationalizing} proposed an approach to help the team decide whether to collect a historical data based on the return on investment.
The authors conducted multiple-case study in seven Agile projects and found that the approach could improve the estimation accuracy.
Tanveer et al.~\cite{tanveer2017utilizing, tanveer2019evaluation} proposed a framework that integrated the change impact analysis to display additional information for effort estimation.
The framework requires the team to provide inputs for the change impact analysis.
Then, it shows the information for effort estimation, i.e., historical data, dependency graph, and impact information.
They integrated the framework to both expert-based and model-based estimation methods~\cite{tanveer2019evaluation}.
They reported that the framework led to a more accurate estimates for both methods.

\underline{\textit{\litrevsupportcatthree{}:}}
Two approaches were proposed to identify the uncertainty in effort estimation.
Grapenthin et al.~\cite{grapenthin2016supporting} proposed an approach that help the team highlight the risks and effort drivers of user stories.
The approach requires the team to manually annotate the user stories using symbols before the effort estimation session.
The author reported that using this approach could improve the shared understanding on the projects, which increased the effort estimation accuracy.
Hannay et al.~\cite{hannay2019agile} proposed a three-points estimation method to illustrate the uncertainty of the estimation of Epics in a project.
In this method, the team have to provide three estimates, i.e., bad, neutral, and good cases.
The then authors used Monte-Carlo simulation on the human-estimated effort of Epics to illustrate the possible outcome of the project's effort.

\begin{tcolorbox}[boxsep=1pt,left=2pt,right=2pt,top=2pt,bottom=2pt]
    \textbf{Findings:} We identified \litrevapproachpaper{} studies proposed the approaches for effort estimation in Agile, which can be categorized based on their purposes and planning levels.
    Regarding the purposes, we observed that the selected studies were proposed to \purposeestimate{} and \purposesupport{} (i.e., \litrevsupportcatonesmall{}, \litrevsupportcattwosmall{}, \litrevsupportcatthreesmall{}).
    Regarding the planning levels, we observed that the majority of the approaches were proposed to be used for sprint planning.
    However, while the majority of these approaches used an automated technique, it is unclear whether they have been evaluated based on the information available during sprint planning or not.
    
    \textbf{Implication:} Prior studies proposed the approaches to \purposeestimate{} and \purposesupport{}.
    However, it is unclear whether these approaches considered the information available during sprint planning or not.
    Using the completed and latest information may not reflect the real usage scenario in each planning level.
    Future work on such approaches should explicitly specify a planning level for the approach and consider the information available in the planning level to mimic the real usage scenarios.
\end{tcolorbox}

==> tables/table_litrev_result_reasons.tex <==
\begin{table}
\caption{Reasons for inaccurate estimation based on the literature (RQ1). The ranks of reasons were retrieved from each study. The alphabet ``x'' indicates that the reason was not ranked by the study. Noted that one study may report multiple reasons in the same rank.}
\label{tab:table_litrev_reasons}
\resizebox{1\linewidth}{!}{
\begin{tabular}{lll}
\hline
\textbf{Reasons}                                                            & \textbf{Ranks} & \textbf{Studies} \\
\hline \hline
\multicolumn{3}{l}{\textbf{R1) Documentation Quality}}                                                           \\
R1.1) Lack of detail or unclear documentation                                & 1,1,2,7,x      & \cite{conoscenti2019combining,sandeep2022effort,usman2018effort,Britto2015,usman2015effort} \\
R1.2) Unstable documentation                                                 & 1,1,1,x        & \cite{sandeep2022effort,usman2018effort,Britto2015,usman2015effort} \\
% R1.3) Poor user stories format                                               & 1,4            & \cite{usman2015effort,sandeep2022effort} \\
R1.3) Error in documentation                                                 & -              & -                \\
\,\, R1.3.1) Mis-documented requirements                                     & 1              & \cite{Britto2015} \\
\,\, R1.3.2) Documented effort error                                         & 4              & \cite{conoscenti2019combining} \\
\hline
\multicolumn{3}{l}{\textbf{R2) Team-related}}                                                            \\
R2.1) Lack of experience of team members                                             & -              & -                \\
\,\, R2.1.1) Lack of experience on the technology or domain knowledge                 & 1,2,3,10      & \cite{conoscenti2019combining,sandeep2022effort,Britto2015,usman2015effort} \\
\,\, R2.1.2) Lack of experience in effort estimation                         & 1,2              & \cite{Britto2015, conoscenti2019combining} \\
\,\, R2.1.3) New or unskilled team members                                    & 3,6,8          & \cite{conoscenti2019combining,sandeep2022effort,usman2015effort} \\
\,\, R2.1.4) Lack of team cohesion                                           & 2              & \cite{Britto2015} \\
R2.2) Insufficient stakeholder participation                                        & -              & -                \\
\,\, R2.2.1) Lack of customers' involvement                                  & 4,8,13       & \cite{sandeep2022effort,Britto2015,usman2015effort} \\
\,\, R2.2.2) Scrum Master not guiding the team                               & 2,12           & \cite{sandeep2022effort,usman2015effort} \\
\,\, R2.2.3) Effort is not estimated by the development team                 & 2              & \cite{Britto2015} \\
R2.3) Knowledge sharing problem                                              & 3,5            & \cite{usman2015effort,sandeep2022effort} \\
R2.4) Dominant personality                                                   & 14             & \cite{sandeep2022effort} \\
\hline
\multicolumn{3}{l}{\textbf{R3) Estimation Practice}}                                                             \\
R3.1) Factors overlooked                                                     & -              & -                \\
\,\, R3.1.1) Side tasks overlooked                                           & 4              & \cite{conoscenti2019combining}  \\
\,\, R3.1.2) Non-functional requirements overlooked                          & 1,3            & \cite{usman2015effort, sandeep2022effort} \\
\,\, R3.1.3) Underestimate the complexity of a function                      & 2,x            & \cite{conoscenti2019combining,usman2018effort} \\
\,\, R3.1.4) Testing effort overlooked                                       & 6,6            & \cite{sandeep2022effort,usman2015effort} \\
\,\, R3.1.5) Technical problems                                              & 8              & \cite{conoscenti2019combining} \\
\,\, R3.1.6) Inaccurately assume that a standard function can be used        & 5              & \cite{conoscenti2019combining} \\
R3.2) Unnecessary work considered                                            & -              & -                \\
\,\, R3.2.1) Unnecessary features considered (gold plating)    & 6              & \cite{conoscenti2019combining} \\
\,\, R3.2.2) Duplicate or Redundancy features considered                     & 3              & \cite{conoscenti2019combining} \\
\,\, R3.3.3) Overestimate the complexity of a function                       & 2,x            & \cite{conoscenti2019combining,usman2018effort} \\
\,\, R3.3.4) Inaccurately assume that a standard function cannot be used     & 5              & \cite{conoscenti2019combining} \\
R3.3) Lack of formal or unstructured estimation process                      & 5,9 and 11           & \cite{usman2015effort,sandeep2022effort} \\
R3.4) Use of fibonacci scale                                                 & x              & \cite{tamrakar2012does} \\
\hline
\multicolumn{3}{l}{\textbf{R4) Project Management}}                                                      \\
R4.1) Overhead due to distributed team settings      & 3,16,x         & \cite{sandeep2022effort,usman2018effort,Britto2015} \\
R4.2) Poor Change Management                                                 & -              & -                \\
\,\, R4.2.1) Scope creep                                                     & 2,8            & \cite{usman2015effort,sandeep2022effort} \\
\,\, R4.2.2) Poor change control                                             & 2,7            & \cite{usman2015effort,sandeep2022effort} \\
R4.3) Poor human-resource management                                         & -              & -                \\
\,\, R4.3.1) Dependence on specific human resource                           & 6,x            & \cite{conoscenti2019combining, usman2018effort} \\
\,\, R4.3.2) Involvement of multiple developers on a story                   & 8              & \cite{conoscenti2019combining} \\
\,\, R4.3.3) Turnover                                                        & -              & -                \\
\,\,\,\, R4.3.3.1) High turnover rate                                        & 2              & \cite{usman2015effort} \\
\,\,\,\, R4.3.3.2) Unexpected turnover                                       & x              & \cite{karna2020effects} \\
\hline
\multicolumn{3}{l}{\textbf{R5) Business Influence}}                                                      \\
R5.1) pressure of timeline                                                   & 10              & \cite{sandeep2022effort} \\
R5.2) Overoptimism due to project bidding pressure                           & 4,5            & \cite{usman2015effort,sandeep2022effort} \\
\hline
\multicolumn{3}{l}{\textbf{R6) Others}}                                                                  \\
R6.1) Rejection of the story                                                 & 5              & \cite{conoscenti2019combining} \\
R6.2) Hardware                                                               & 15             & \cite{sandeep2022effort} \\
\hline
\end{tabular}
}
\end{table}
